FaithformBench: Benchmarking Faithfulness of Mathematical Chain-of-Thought Autoformalisation

Autoformalisation (AF) systems map natural language reasoning steps into formal statements in a proof assistant such as Lean. We consider how to assess the faithfulness of these systems. Existing approaches require expensive human-annotated ground truth, or rely on LLM judges or embedding models, which come with limited guarantees of accuracy. In addition, these methods typically only consider inputs that are known to be correct, and therefore do not assess whether the AF translates incorrect inputs faithfully. To address these limitations, we propose a new benchmark for AF faithfulness that is cheap to apply, sound under weak assumptions, and assesses both positive and negative examples. Our method is based on automatically generating perturbed reasoning steps that are designed to be invalid, and then measuring validity preservation on unperturbed steps and invalidity preservation on perturbed steps. We apply our method to eight AF systems across four mathematical datasets, and observe pervasive sycophancy: many AFs "silently correct" invalid inputs into provable statements. The most validity-preserving fine-tuned AFs are also the most sycophantic, suggesting a tension between validity and invalidity preservation in current AF systems.

==> Images/diagram/step1_processbench.tex <==
%
\begin{minipage}[t][2.6cm][t]{\linewidth}
    \centering
    \textbf{\strut\footnotesize ProcessBench (NL)}\\[0.1em]
    \textit{\tiny ID: gsm8k-216}\\[0.2em]

    {
        \tiny\sffamily
        \begin{flushleft}
            \setlength{\baselineskip}{1.4em}
            \textbf{[$S_1$]} Mon rain $= 2$.\\
            \textbf{[$S_2$]} $2\times$Mon $= 4$.\\
            \textbf{[$S_3$]} Tue $=$ ($2\times$Mon) $+ 1$.\\
            \textbf{[$S_4$]} Tue $= 4 + 1$.\\
            \textbf{[$S_5$]} Tue $= 5$.
        \end{flushleft}
    }
\end{minipage}


==> Images/diagram/step3_perturbation.tex <==
%
\begin{minipage}[t][2.6cm][t]{\linewidth}
    \centering
    \textbf{\strut\footnotesize Perturbation}\\[0.2em]

    {
        \tiny\sffamily
        \setlength{\parskip}{0em}
        \color{black}

        %
        \begin{minipage}[t]{0.46\linewidth}
            \centering
            \textcolor{gray}{-- Unperturbed}\\[0.2em]
            [$S_4$] Tue $= 4 + 1$\\[0.2em]
            \begin{tikzpicture}[
                baseline=(current bounding box.center),
                dag_node/.style={
                    circle, draw=black!70, fill=white, thick,
                    minimum size=1em, inner sep=0.3pt,
                    font=\sffamily\tiny\bfseries
                },
                dag_edge/.style={->, >=Latex, semithick, color=black!60}
            ]
                \node[dag_node] (a4) {$S_4$};
                \node[dag_node, above left=0.32cm and 0.08cm of a4] (a2) {$S_2$};
                \node[dag_node, above right=0.32cm and 0.08cm of a4] (a3) {$S_3$};
                \draw[dag_edge] (a2) -- (a4);
                \draw[dag_edge] (a3) -- (a4);
            \end{tikzpicture}
        \end{minipage}%
        \hfill%
        \color{gray}\vrule width 0.4pt\color{black}%
        \hfill%
        %
        \begin{minipage}[t]{0.46\linewidth}
            \centering
            \textcolor{gray}{-- Perturbed}\\[0.2em]
            [$S'_4$] Tue $= 4$ \textcolor{orange!90!black}{$/\, 2$}\\[0.2em]
            \begin{tikzpicture}[
                baseline=(current bounding box.center),
                dag_node/.style={
                    circle, draw=black!70, fill=white, thick,
                    minimum size=1em, inner sep=0.3pt,
                    font=\sffamily\tiny\bfseries
                },
                perturbed_node/.style={
                    dag_node, draw=orange!90!black, fill=orange!20, line width=1pt
                },
                dag_edge/.style={->, >=Latex, semithick, color=black!60}
            ]
                \node[perturbed_node] (b4) {$S'_4$};
                \node[dag_node, above left=0.32cm and 0.08cm of b4] (b2) {$S_2$};
                \node[dag_node, above right=0.32cm and 0.08cm of b4] (b3) {$S_3$};
                \draw[dag_edge] (b2) -- (b4);
                \draw[dag_edge] (b3) -- (b4);
            \end{tikzpicture}
        \end{minipage}
    }
\end{minipage}


==> Images/diagram/step4_formalisation.tex <==
%
\begin{minipage}[t][2.6cm][t]{\linewidth}
    \centering
    \textbf{\strut\footnotesize Formalisation}\\[0.1em]

    \begin{minipage}{\linewidth}
        \tiny\ttfamily
        \setlength{\parskip}{0em}
        \linespread{0.95}\selectfont
        \color{blue!40!black}

        %
        \begin{minipage}[t]{0.47\linewidth}
            \raggedright
            \textcolor{gray}{-- Perturbed}\\
            \textcolor{gray}{-- Direct}\\
            \textcolor{black}{theorem rain\_bad}\\
            \ (mon := 2)\\
            \ (tue := 2*mon+1)\\
            \ : tue = 4/2\\
            \ := by \textcolor{gray}{sorry}
        \end{minipage}%
        \hfill%
        \color{gray}\vrule width 0.4pt\color{blue!40!black}%
        \hfill%
        %
        \begin{minipage}[t]{0.47\linewidth}
            \raggedright
            \textcolor{gray}{-- Perturbed}\\
            \textcolor{gray}{-- Negation}\\
            \textcolor{black}{theorem rain\_not}\\
            \ : \textcolor{red!80!black}{$\lnot$ ($\forall$ \textcolor{gray}{\ldots},}\\
            \ \ \ \ \ tue = 4/2\textcolor{red!80!black}{)}\\
            \ := by \textcolor{gray}{sorry}
        \end{minipage}
    \end{minipage}
\end{minipage}


==> Images/diagram/step5_proved.tex <==
%
\begin{minipage}[t][2.6cm][t]{\linewidth}
    \centering
    \textbf{\strut\footnotesize Proof}\\[0.1em]

    \begin{minipage}{\linewidth}
        \tiny\ttfamily
        \setlength{\parskip}{0em}
        \linespread{0.95}\selectfont
        \color{blue!40!black}

        %
        \begin{minipage}[t]{0.47\linewidth}
            \raggedright
            \textcolor{gray}{-- Perturbed}\\
            \textcolor{gray}{-- Direct}\\
            \textcolor{black}{... := by}\\
            \ simp\\
            \ rfl\\
            \ \textcolor{red!60!black}{-- Failed}\\
            \ \textcolor{yellow!60!black}{-- (Expected)}
            
        \end{minipage}%
        \hfill%
        \color{gray}\vrule width 0.4pt\color{blue!40!black}%
        \hfill%
        %
        \begin{minipage}[t]{0.47\linewidth}
            \raggedright
            \textcolor{gray}{-- Perturbed}\\
            \textcolor{gray}{-- Negation}\\
            \textcolor{black}{... := by}\\
            \ intro h\\
            \ have : $5\neq 2$\\
            \ \ := by decide\\
            \ \textcolor{green!60!black}{-- \checkmark Proved}
        \end{minipage}
    \end{minipage}
\end{minipage}

